Hybrid Asymmetric Linear Higgs Factory (HALHF) interim progress report (Pre-CDR)

This document reports on the current status of the HALHF project, as an intermediate step towards a full Conceptual Design Report (CDR). After defining the structure of the project and the current baseline, the document details progress with physics studies, where substantial progress has been made both in understanding the beam--beam interaction for asymmetric collisions and its effects on the design of the interaction region. Representative physics processes have been considered, for which HALHF performs almost as well as a symmetric collider. Progress on the plasma linac is reported, including achromatic staging optics, simulations of several HALHF cells staged together and a simplified simulation of the full 48-cell accelerator. Studies of the transverse instability and tolerances are presented. Polarisation can be preserved during the acceleration process. The design of a suitable plasma cell and cooling is underway. The radiation environment and transport to the beam dumps represent a challenge. A scheme to distribute drivers to the PWFA cells is detailed. The polarised positron and electron sources are outlined. Finally, new ideas on the beam-delivery system are shown. The final section outlines the strategy for future work and estimates the resources required to produce a full CDR.

==> driver_guiding_and_field_sketch.tex <==





% Into-the-page current symbol
\newcommand{\intothepage}[2]{
    \draw[draw=blue!70, fill=blue!15, thick, opacity=0.5] (#1,#2) circle (4.5pt);
    \draw[thick, blue!70, opacity=0.5] (#1-0.08,#2-0.08) -- (#1+0.08,#2+0.08);
    \draw[thick, blue!70, opacity=0.5] (#1-0.08,#2+0.08) -- (#1+0.08,#2-0.08);
}

\tikzstyle{axis}=[dashed, gray!80, line width=0.8pt]
\tikzstyle{mainaxis}=[-{Stealth[length=3mm, width=2mm]}, thick, black]
\tikzstyle{electron}=[circle, fill=blue!70!black, inner sep=0.8pt]
\tikzstyle{ion}=[circle, fill=red!70, opacity=0.5, inner sep=1.2pt]
\tikzstyle{currentline}=[{Stealth[length=3mm, width=2mm]}-, thick, blue!45, opacity=0.45]
\tikzstyle{currenttext}=[blue!45, opacity=0.8, font=\normalfont]


\centering
    % -------------------------------------------------------------------------
    % LEFT MINIPAGE: DIAGRAM A
    % -------------------------------------------------------------------------
    \begin{minipage}[b]{0.90\columnwidth}
    \centering
    \begin{tikzpicture}[>=Stealth, scale=0.7, every node/.style={scale=0.7}]

        %\useasboundingbox (-5.8, -3.2) rectangle (5.8, 3.2);

        \coordinate (CenterPoint) at (0,0); 
        \coordinate (FlatRef) at (3.5,0);
        \coordinate (TiltRef) at (8:3.5); % 8°

        % s–axis
        \draw[mainaxis] (-4.5,0) -- (4.5,0) node[above, black, font=\Large] {$s$};

        % Current lines
        \draw[currentline] (-4.5,  2.5) -- (4.5,  2.5);
        \draw[currentline] (-4.5,  1.7) -- (4.5,  1.7);
        \draw[currentline] (-4.5,  0.9) -- (4.5,  0.9);
        \draw[currentline] (-4.5, -0.9) -- (4.5, -0.9);
        \draw[currentline] (-4.5, -1.7) -- (4.5, -1.7);
        \draw[currentline] (-4.5, -2.5) -- (4.5, -2.5);

        \node[currenttext, anchor=east, font=\large] at (-4.6,  2.5) {Current};
        %\node[currenttext, anchor=east] at (-4.6, -2.5) {Current};

        % Background ions
        \foreach \x in {-4.0, -3.1, ..., 4.0} {
            \foreach \y in {-2.0, -1.0, 0, 1.0, 2.0} {
                \node[ion] at (\x + 0.2*rand, \y + 0.1*rand) {};
            }
        }

        % Tilted system
        \begin{scope}[rotate=8]
            % Tilted dashed center line
            \draw[-{Stealth[length=3mm, width=2mm]}, black, line width=0.8pt, dashed] 
                (-4.5,0) -- (4.5,0);

            % Blowout bubble (this defines the geometry)
            \begin{scope}
                \clip (-3.5,-1.8) rectangle (3.5,1.8);
                \fill[red!5, draw=blue!40!gray, thick, dashed] 
                    (2.2,0) .. controls (1.9,1.3) and (-0.5,1.4) .. (-1.3,0)
                            .. controls (-0.5,-1.4) and (1.9,-1.3) .. (2.2,0);
            \end{scope}

            % ------------------------------------------------------------------
            % Plasma electrons: placed ON THE SAME GEOMETRY as the blowout
            % bubble, i.e. directly on that dashed blue curve.
            % We sample the same parametric shape with several t–values.
            % ------------------------------------------------------------------
            \foreach \t in {0,0.05,...,1} {
                % Forward part (from 2.2,0 up to -1.3,0 via upper controls)
                \pgfmathsetmacro{\xA}{2.2}
                \pgfmathsetmacro{\yA}{0}
                \pgfmathsetmacro{\xB}{1.9}
                \pgfmathsetmacro{\yB}{1.3}
                \pgfmathsetmacro{\xC}{-0.5}
                \pgfmathsetmacro{\yC}{1.4}
                \pgfmathsetmacro{\xD}{-1.3}
                \pgfmathsetmacro{\yD}{0}
                % Cubic Bezier interpolation for upper half
                \pgfmathsetmacro{\xu}{
                    (1-\t)^3*\xA +
                    3*(1-\t)^2*\t*\xB +
                    3*(1-\t)*\t^2*\xC +
                    \t^3*\xD
                }
                \pgfmathsetmacro{\yu}{
                    (1-\t)^3*\yA +
                    3*(1-\t)^2*\t*\yB +
                    3*(1-\t)*\t^2*\yC +
                    \t^3*\yD
                }

                % Return part (from -1.3,0 back to 2.2,0 via lower controls)
                \pgfmathsetmacro{\xE}{-1.3}
                \pgfmathsetmacro{\yE}{0}
                \pgfmathsetmacro{\xF}{-0.5}
                \pgfmathsetmacro{\yF}{-1.4}
                \pgfmathsetmacro{\xG}{1.9}
                \pgfmathsetmacro{\yG}{-1.3}
                \pgfmathsetmacro{\xH}{2.2}
                \pgfmathsetmacro{\yH}{0}
                \pgfmathsetmacro{\xl}{
                    (1-\t)^3*\xE +
                    3*(1-\t)^2*\t*\xF +
                    3*(1-\t)*\t^2*\xG +
                    \t^3*\xH
                }
                \pgfmathsetmacro{\yl}{
                    (1-\t)^3*\yE +
                    3*(1-\t)^2*\t*\yF +
                    3*(1-\t)*\t^2*\yG +
                    \t^3*\yH
                }

                % Small jitter so dots are not perfectly regular
                \pgfmathsetmacro{\jx}{0.001*(2*rand-1)}
                \pgfmathsetmacro{\jy}{0.001*(2*rand-1)}

                % Electron on upper branch
                \node[electron, opacity=0.9] at ({\xu+\jx},{\yu+\jy}) {};
                % Electron on lower branch
                \node[electron, opacity=0.9] at ({\xl+\jx},{\yl+\jy}) {};
            }

            % Particle bunches
            \fill[orange!90!black, opacity=1.0] (2.2,0) ellipse (0.55cm and 0.22cm);
            \fill[blue!70!black, opacity=0.9] (-0.7,0) ellipse (0.25cm and 0.11cm);
        \end{scope}

        % Lab axes
        \coordinate (Origin) at (-3.8,0);
        \fill[black] (Origin) circle (1.5pt);
        \draw[mainaxis] (Origin) -- ($(Origin) + (1.2, 0)$) node[above, black, font=\Large] {$z$};
        \draw[mainaxis] (Origin) -- ($(Origin) + (0, 1.2)$) node[above, black, font=\Large] {$y$};

        % Angle marker
        \pic [draw, ->, "$y'$", angle radius=3.0cm, angle eccentricity=1.15, font=\large] 
            {angle = FlatRef--CenterPoint--TiltRef};

    \end{tikzpicture}
    \\ \textbf{(a)}
    \end{minipage}%
    %\hspace{0.12\textwidth}
    \vspace{1em}
    
    % -------------------------------------------------------------------------
    % RIGHT MINIPAGE: DIAGRAM B
    % -------------------------------------------------------------------------
    \begin{minipage}[b]{0.99\columnwidth}
    \centering
    \begin{tikzpicture}[>=Stealth, scale=0.7, every node/.style={scale=0.7}]
        %\useasboundingbox (-4.0, -2.8) rectangle (5.5, 3.2);
        
        \tikzstyle{sideaxis}=[-{Stealth[length=3mm, width=2mm]}, thick, black]

        % Coordinate axes
        \coordinate (SideOrigin) at (0,0);
        \draw[line width=3.5pt, white, opacity=0.8] (-2.8,0) -- (2.8,0);
        \draw[line width=3.5pt, white, opacity=0.8] (0,-2.4) -- (0,2.4);

        \draw[sideaxis] (-2.8,0) -- (2.8,0) node[right, font=\Large] {$x$};
        \draw[sideaxis] (0,-2.4) -- (0,2.4) node[above, font=\Large] {$y$};
        \fill[black] (SideOrigin) circle (1.5pt);
        
        % Place ions
        \foreach \x in {-2.5, -1.5, ..., 2.5} {
            \foreach \y in {-2.0, -1.0, 0, 1.0, 2.0} {
                \node[ion] at (\x + 0.15*rand, \y + 0.15*rand) {};
            }
        }

        % Current lines into the page
        \foreach \x in {-2.0, -1.0, 0.0, 1.0, 2.0} {
            \foreach \y in {-1.5, -0.5, 0.5, 1.5} {
                \intothepage{\x}{\y}
            }
        }

        % Labels
        \node[currenttext, anchor=west, font=\large] at (3.8, 1.5) {Current:};
        \begin{scope}
            \intothepage{5.7}{1.5}
        \end{scope}
        
        \node[green!60!black, font=\normalfont, anchor=west, font=\Large] 
            at (3.8, 0.9) {$\bm{B}_\text{ext}$: };
        \draw[
            -{Stealth[length=3mm,width=2mm]},
            green!60!black,
            thick
        ] (5.1,0.9) -- (5.8,0.9);

        % Magnetic field lines
        \foreach \r in {0.70, 1.35, 2.00} {
            \pgfmathsetmacro{\w}{\r * 1.5}
        
            % Full circle
            \draw[
                draw=green!60!black,
                line width=0.5*\w pt,
                opacity=0.85
            ] (0,0) circle (\r cm);
        
            % Short arc with arrowhead
            \draw[
                -{Stealth[length=\w*2.5pt, width=\w*1.5pt]},
                green!60!black,
                opacity=0.85,
                line width=0.5*\w pt
            ]
            (60:\r) arc (60:30:\r);
        }
        
    \end{tikzpicture}
    \\ \textbf{(b)}
    \end{minipage}

%\caption{\textbf{(a)} The driver-guiding can be implemented using a uniform current flowing along the reference trajectory. \textbf{(b)} The current sets up an azimuthal magnetic field $B_\text{ext}$, generating a radial focusing field, steering the driver back to the axis.}


